Actuator-Constrained Reinforcement Learning for High-Speed Quadrupedal Locomotion

This paper presents a method for achieving high-speed running of a quadruped robot by considering the actuator torque-speed operating region in reinforcement learning. The physical properties and constraints of the actuator are included in the training process to reduce state transitions that are infeasible in the real world due to motor torque-speed limitations. The gait reward is designed to distribute motor torque evenly across all legs, contributing to more balanced power usage and mitigating performance bottlenecks due to single-motor saturation. Additionally, we designed a lightweight foot to enhance the robot's agility. We observed that applying the motor operating region as a constraint helps the policy network avoid infeasible areas during sampling. With the trained policy, KAIST Hound, a 45 kg quadruped robot, can run up to 6.5 m/s, which is the fastest speed among electric motor-based quadruped robots.

==> packages/model_citation_influence.tex <==
% model_citation_influence.tex
%
% Copyright (C) 2010,2011 Laura Dietz
% Copyright (C) 2012 Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Citation influence model
% Cite this model as 
% Laura Dietz, Steffen Bickel, Tobias Scheffer. 
% Unsupervised Prediction of Citation Influences. 
% In: Proceedings of International Conference on Machine Learning. 2007

%\beginpgfgraphicnamed{model-citation-influence}
\begin{tikzpicture}

  % Layout the variables
  \matrix[row sep=0.5cm, column sep=1.2cm] (LDA)
  { %
    & %
    & %
    \node[latent] (gamma)  {$\gamma$} ; & %
    \node[latent] (lambda) {$\lambda$} ; & %
    \node[latent] (psi)    {$\psi$} ; %
    \\
    \\
    \node[latent] (theta)  {$\theta$} ; & %
    & %
    \node[latent] (C)      {$C$} ; & %
    \node[latent] (S)      {$S$} ; & %
    \\
    & %
    & %
    \factor       {T-f1}   {Multi} {} {}; & %
    & %
    \factor       {T-f2}   {below:Multi} {} {}; & %
    \\
    \node[latent] (T')     {$T'$} ; & %
    & %
    \node[latent] (T)      {$T$} ; & %
    \\
    \factor       {W'-f}   {Multi} {} {}; & %
    \node[latent] (phi)    {$\phi$} ; & %
    \factor       {W-f}    {Multi} {} {}; %
    \\
    \node[obs] (W')        {$W'$} ; & %
    & %
    \node[obs] (W)         {$W$} ;
    \\
  };

  % Remaining factors
  \factor[above=of T']     {T'-f}     {left:Multi} {} {}; %
  \factor[above=of theta]  {theta-f}  {left:Dir} {} {}; %
  \factor[above=of C]      {C-f}      {left:Multi} {} {}; %
  \factor[above=of S]      {S-f}      {left:Bern} {} {}; %
  \factor[above=of gamma]  {gamma-f}  {left:Dir} {} {}; %
  \factor[above=of lambda] {lambda-f} {left:Beta} {} {}; %
  \factor[above=of psi]    {psi-f}    {left:Dir} {} {}; %
  \factor[above=of phi]    {phi-f}    {left:Dir} {} {}; %

  % Hyperparameters
  \node[const, above=of theta]  (atheta)  {$\alpha_\theta$}; %
  \node[const, above=of phi]    (aphi)    {$\alpha_\phi$}; %
  \node[const, above=of gamma]  (agamma)  {$\alpha_\gamma$}; %
  \node[const, above=of lambda, xshift=-0.5cm] (alambda1)
  {$\alpha_{\lambda_\theta}$}; %
  \node[const, above=of lambda, xshift=0.5cm] (alambda2)
  {$\alpha_{\lambda_\psi}$}; %
  \node[const, above=of psi]    (apsi)    {$\alpha_\psi$}; %

  % Factor connections
  \factoredge {phi}               {W'-f}     {W'} ; %
  \factoredge {phi}               {W-f}      {W} ; %
  \factoredge {theta}             {T'-f}     {T'} ; %
  \factoredge {theta}             {T-f1}     {T} ; %
  \factoredge {psi}               {T-f2}     {T} ; %
  \factoredge {atheta}            {theta-f}  {theta} ; %
  \factoredge {gamma}             {C-f}      {C} ; %
  \factoredge {lambda}            {S-f}      {S} ; %
  \factoredge {agamma}            {gamma-f}  {gamma} ; %
  \factoredge {alambda1,alambda2} {lambda-f} {lambda} ; %
  \factoredge {apsi}              {psi-f}    {psi} ; %
  \factoredge {aphi}              {phi-f}    {phi} ; %

  % Gates
  \gate {W'-gate} {(W'-f)(W'-f-caption)} {T'} ; %
  \gate {W-gate}  {(W-f)(W-f-caption)}   {T} ; %
  \gate {T-gate}  {(T-f1)(T-f1-caption)} {C} ;
  \vgate {T-vgate} %
  {(T-gate)} {$S=0$} %
  {(T-f2)(T-f2-caption)} {$S=1$} %
  {S} ; %

  % Plates
  \plate {LDA1} { %
    (T')(T'-f)(T'-f-caption) %
    (W')(W'-gate) %
  } {$\forall w' \in c$} ; %

  \plate {LDA2} { %
    (LDA1) %
    (theta)(theta-f)(theta-f-caption) %
  } {$\forall c \in \mathcal{C}$} ; %

  \plate {} { %
    (phi)(phi-f)(phi-f-caption) %
  } {$\forall t \in \mathcal{T}$} ; %

  \plate {P1} { %
    (W)(W-gate) %
    (T)(T-vgate) %
    (C)(C-f)(C-f-caption) %
    (S)(S-f)(S-f-caption) %
  } {$\forall w \in d$} ;

  \plate {} { %
    (P1) %
    (gamma)(gamma-f)(gamma-f-caption) %
    (lambda)(lambda-f)(lambda-f-caption) %
    (psi)(psi-f)(psi-f-caption) %
  } {$\forall d \in \mathcal{D}$} ; %

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 


==> packages/model_lda.tex <==
% model_lda.tex
%
% Copyright (C) 2010,2011 Laura Dietz
% Copyright (C) 2012 Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Latent Diriclet allocation model

%\beginpgfgraphicnamed{model-lda}
\begin{tikzpicture}[x=1.7cm,y=1.8cm]

  % Nodes

  \node[obs]                   (X)      {$X$} ; %
  \node[latent, above=of X]    (T)      {$T$} ; %
  \node[latent, above=of T]    (theta)  {$\theta$}; %
  \node[const, above=of theta] (atheta) {$\alpha_\theta$};


  % Factors
  \factor[above=of X]     {X-f}     {Multi} {} {} ; %
  \factor[above=of T]     {T-f}     {left:Multi} {} {} ; %
  \factor[above=of theta] {theta-f} {left:Dir} {} {} ; %

  % More nodes
  \node[latent, right=of X-f] (phi)  {$\phi$}; %
  \node[const, above=of phi]  (aphi) {$\alpha_\phi$}; %

  \factor[above=of phi] {phi-f} {right:Dir} {} {} ; %

  \factoredge {theta}  {T-f}     {T} ; %
  \factoredge {atheta} {theta-f} {theta} ; %
  \factoredge {phi}    {X-f}     {X} ; %
  \factoredge {aphi}   {phi-f}   {phi} ; %

  \gate {X-gate} {(X-f)(X-f-caption)} {T}

  \plate {plate1} { %
    (X)(X-gate) %
    (T)(T-f)(T-f-caption) %
  } {$\forall 1 \leq i \leq n_d$}; %
  \plate {} { %
    (plate1) %
    (theta)(theta-f)(theta-f-caption) %
  } {$\forall d \in \mathcal{D}$} ; %
  \plate {} { %
    (phi)(phi-f)(phi-f-caption) %
  } {$\forall t \in \mathcal{T}$} ; %

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 


==> packages/model_pca.tex <==
% model_pca.tex
%
% Copyright (C) 2012 Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% PCA model

%\beginpgfgraphicnamed{model-pca}
\begin{tikzpicture}

  % Define nodes
  \node[obs]                               (y) {$y$};
  \node[latent, above=of y, xshift=-1.2cm] (w) {$\mathbf{w}$};
  \node[latent, above=of y, xshift=1.2cm]  (x) {$\mathbf{x}$};
  \node[latent, right=2cm of y]            (t) {$\tau$};

  % Connect the nodes
  \edge {x,w,t} {y} ; %

  % Plates
  \plate {yx} {(x)(y)} {$N$} ;
  \plate {} {(w)(y)(yx.north west)(yx.south west)} {$M$} ;

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 


==> packages/model_pca2.tex <==
% model_pca2.tex
%
% Copyright (C) 2010,2011 Laura Dietz
% Copyright (C) 2012 Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% PCA model

%\beginpgfgraphicnamed{model-pca}
\begin{tikzpicture}

  % Define nodes

  % Y
  \node[obs]          (y)   {$y$}; %
  \factor[above=of y] {y-f} {left:$\mathcal{N}$} {} {} ; %

  % W and X
  \node[det, above=of y]            (dot) {dot} ; % 
  \node[latent, above left=1.2 of dot]  (w)   {$\mathbf{w}$}; %
  \node[latent, above right=1.2 of dot] (x)   {$\mathbf{x}$}; %

  % W hyperparameters
  \node[const, above=1.2 of w, xshift=-0.5cm] (mw) {$\mu_w$} ; %
  \node[const, above=1.2 of w, xshift=0.5cm]  (aw) {$\alpha_w$} ; %

  % X hyperparameters
  \node[const, above=1.2 of x, xshift=-0.5cm] (mx) {$\mu_x$} ; %
  \node[const, above=1.2 of x, xshift=0.5cm]  (ax) {$\alpha_x$} ; %

  % noise
  \node[latent, right=2.5cm of y-f]         (t)   {$\tau$}; %
  \node[const, above=of t, xshift=-0.5cm] (at)  {$\alpha_\tau$} ; %
  \node[const, above=of t, xshift=0.5cm]  (bt)  {$\beta_\tau$} ; %

  % Factors
  \factor[above=of w] {w-f} {left:$\mathcal{N}$} {mw,aw} {w} ; %
  \factor[above=of x] {x-f} {left:$\mathcal{N}$} {mx,ax} {x} ; %
  \factor[above=of t] {t-f} {left:$\mathcal{G}$} {at,bt} {t} ; %
  \factoredge {dot,t} {y-f} {y} ; %

  % Connect w and x to the dot node
  \edge[-] {w,x} {dot} ;

  % Plates
  \plate {yx} { %
    (y)(y-f)(y-f-caption) %
    (x)(x-f)(x-f-caption) %
    (dot) %
  } {$N$} ;
  \plate {} {%
    (y)(y-f)(y-f-caption) %
    (w)(w-f)(w-f-caption) %
    (dot) %
    (yx.north west)(yx.south west) %
  } {$M$} ;

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 



==> packages/tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

